AIT-QA: Question Answering Dataset over Complex Tables in the Airline Industry

Recent advances in transformers have enabled Table Question Answering (Table QA) systems to achieve high accuracy and SOTA results on open domain datasets like WikiTableQuestions and WikiSQL. Such transformers are frequently pre-trained on open-domain content such as Wikipedia, where they effectively encode questions and corresponding tables from Wikipedia as seen in Table QA dataset. However, web tables in Wikipedia are notably flat in their layout, with the first row as the sole column header. The layout lends to a relational view of tables where each row is a tuple. Whereas, tables in domain-specific business or scientific documents often have a much more complex layout, including hierarchical row and column headers, in addition to having specialized vocabulary terms from that domain. To address this problem, we introduce the domain-specific Table QA dataset AIT-QA (Airline Industry Table QA). The dataset consists of 515 questions authored by human annotators on 116 tables extracted from public U.S. SEC filings (publicly available at: https://www.sec.gov/edgar.shtml) of major airline companies for the fiscal years 2017-2019. We also provide annotations pertaining to the nature of questions, marking those that require hierarchical headers, domain-specific terminology, and paraphrased forms. Our zero-shot baseline evaluation of three transformer-based SOTA Table QA methods - TaPAS (end-to-end), TaBERT (semantic parsing-based), and RCI (row-column encoding-based) - clearly exposes the limitation of these methods in this practical setting, with the best accuracy at just 51.8\% (RCI). We also present pragmatic table preprocessing steps used to pivot and project these complex tables into a layout suitable for the SOTA Table QA models.

==> outline.tex <==
\section*{Outline}

\begin{itemize}
    \item Introduction
    \begin{itemize}
        \item Show example of table-question pair, highlighting:
        \begin{itemize}
            \item domain-specific vocabulary
            \item column header hierarchy
            \item row header hierarchy
        \end{itemize}
        \item Explain novelty:
        \begin{itemize}
            \item Domain-specific dataset
            \item Complex table structure
        \end{itemize}
    \end{itemize}
    \item Approach
    \begin{itemize}
        \item High-level overview of dataset
        \item Describe annotation process
        \item Summarize differences from existing datasets:
        \begin{itemize}
            \item WikiTableQuestions
            \item WikiSQL
        \end{itemize}
    \end{itemize}
    \item Evaluation and Analysis
    \begin{itemize}
        \item Evaluate performance of SOTA TableQA models on benchmark dataset (what should be dataset these models are trained on?):
        \begin{itemize}
            \item RCI
            \item TaBERT \cite{tabert}
            \item TAPAS \cite{tapas}
        \end{itemize}
        \item Explore which question-table pairs are harder for SOTA models, by evaluating them on different slices:
        \begin{itemize}
            \item Entire dataset
            \item Questions depending on row header hierarchy
            \item KPI vs Table-driven questions
            \item Term matches with question and tables vs not
            \item BERT finetuning with text vs no.
            \item Using KPI descriptions vs not.
            \item more tricks to deal with hierarchical headers.
        \end{itemize}
        \item Demonstrate how performance of existing models (not trained on row headers) can be improved through transposing.
        \item Identify questions where all SOTA systems fail and find/discuss commonalities
    \end{itemize}
\end{itemize}
